Operator theory of electrical resistance networks

A resistance network is a weighted graph $(G,c)$ with intrinsic (resistance) metric $R$. We embed the resistance network into the Hilbert space ${\mathcal H}_{\mathcal E}$ of functions of finite energy. We use the resistance metric to study ${\mathcal H}_{\mathcal E}$, and vice versa and show that the embedded images of the vertices $\{v_x\}$ form a reproducing kernel for this Hilbert space. We also obtain a discrete version of the Gauss-Green formula for resistance networks and show that resistance networks which support nonconstant harmonic functions of finite energy have a certain type of \emph{boundary}. We obtain an analytic boundary representation for the harmonic functions of finite energy in a sense analogous to the Poisson or Martin boundary representations, but with different hypotheses, and for a different class of functions. In the process, we construct a dense space of "smooth" functions of finite energy and obtain a Gel'fand triple for ${\mathcal H}_{\mathcal E}$. This allows us to represent the resistance network as a system of Gaussian random variables indexed by vertices. We also study the spectral representation for $\Delta$ on ${\mathcal H}_{\mathcal E}$ and show how nonzero defect entails a nontrivial boundary. All of the above are are detected by the operator theory of ${\mathcal H}_{\mathcal E}$ but not $\ell^2$. Our results apply to the Heisenberg model for the isotropic ferromagnet, improving earlier results of R. T. Powers on the problem of long-range order (in reference to KMS states on the $C^\ast$-algebra of the model).

==> fundamentals.tex <==
%%!TEX root = OTERN.tex

\setcounter{chapter}{-1}

\chapter{Fundamentals and preliminaries}
\label{sec:Fundamentals-and-preliminaries}

The magic of Hilbert space resides in the following innocent-looking axioms:
\begin{enumerate}
  \item A complex vector space \sH.
  \item A complex-valued function on $\sH \times \sH$, denoted by $\la \cdot,\cdot\ra$ and satisfying
  \begin{enumerate}[(a)]
    \item For every $v \in \sH$, $\la v, \cdot\ra : \sH \to \bC$ is linear.
    \item For every $v_1,v_2 \in \sH$, $\la v_1,v_2\ra = \cj{\la v_2,v_1\ra}$.
    \item For every $v \in \sH$, $\la v,v\ra \geq 0$, with equality if and only if $v=0$.
  \end{enumerate}
  \item Under the norm defined by $\|v\|_\sH := \la v,v\ra^{1/2}$, \sH is complete.
\end{enumerate}

\begin{exm}[Square-summable sequences]
  For a \bC-valued function $v$ on the integers, let $\|v\|_2 := \left(\sum_{n \in \bZ} |v(n)|^2\right)^{1/2}$. Then
  \[\ell^2(\bZ) := \{v:\bZ \to \bC \suth \|v\|_2 < \iy\}\]
  is a Hilbert space.
\end{exm}

\begin{exm}[Classical $L^2$-spaces]
  For a measurable \bC-valued function $v$ on a measure space $(X,\gm)$, let $\|v\|_2 := \left(\int_X |v(x)|^2 \,d\gm(x) \right)^{1/2}$. Then
  \[L^2(\gm) := \{v:X \to \bC \suth \|v\|_2 < \iy\}\]
  is a Hilbert space.
\end{exm}
